Flexible Content Placement in Cache Networks using Reinforced Counters

In this paper we study the problem of content placement in a cache network. We consider a network where routing of requests is based on random walks. Content placement is done using a novel mechanism referred to as reinforced counters. To each content we associate a counter, which is incremented every time the content is requested, and which is decremented at a fixed rate. We model and analyze this mechanism, tuning its parameters so as to achieve desired performance goals for a single cache or for a cache network. We also show that the optimal static content placement, without reinforced counters, is NP hard under different design goals.

==> discussion.tex <==
\subsection{Discussion}
\label{sec:assum}

In this section we discuss some of our model assumptions.

\begin{itemize}
\item \emph{lack of stable custodians}: in this paper we assume that every content is placed in at least one cache.
  Having one replica of each content in at least one cache is key to guarantee content \emph{persistence}, in case custodians
are unstable. As in peer-to-peer systems, publisher willing to reduce energy and bandwidth costs can leave 
the network if replicas of the files are available
in the network.
\item \emph{space constrained system}: we assume that not all caches can store replicas of all the files that circulate in the network.
 This assumption holds since caches are placed on top of routers, and core routers are shared among many users.
\item \emph{separation between control plane and data plane}: in this paper we assume separation between the control plane
and the data plane.  Juniper already implements separation between data and control planes in its routers. In addition, virtual machines
 can be used to implement services on top of such routers~\cite{juniper}.
\end{itemize}


==> eval.tex <==
\section{Evaluation} \label{sec:eval}

TO BE DONE: show many numerical examples of solutions of the MICQ program

TO BE DONE: try to come up with heuristics

TO BE DONE: consider more general scenarios (e.g., when we have cost to FIND file in cache)

TO BE DONE: consider the followig topologies under Zipf workload 

\begin{itemize}
\item tree: hierarchy
\item ring: Rede Rio, RNP (MANET) 
\item star: local connections
\end{itemize}

TO BE DONE: get topologies with Bernardo


==> mix.tex <==

\section{Mixed Integer Quadratically Constrained Program Formulation} \label{lp}

Given the exogenous arrival rates $\lambda_{ij}$, $1 \leq i \leq C$, $1 \leq j \leq F$,  and the routing matrix $M$, our goal is to find 
the optimal content placement, i.e., to compute $A_{ij}$, $1 \leq i \leq C$, $1 \leq j \leq F$.   To this aim, we must solve the following
mixed integer quadratically constrained program,
\begin{eqnarray}
\ensuremath{\mbox{\sc PlacementProblem:}} \min && \sum_{i=1}^C \alpha_i \label{eqgoal} \\
\text{subject to} && \nonumber \\
\sum_{i=1}^{C} A_{ij}& \ge & 1, \quad j=1, \ldots, F \label{eq1set} \\
\sum_{j=1}^{F} A_{ij}& \le & s_i, \quad i=1, \ldots, C  \label{eq2set}  \\
\alpha_i &=& \sum_{j=1}^F \alpha_{ij}, \qquad \alpha_{i} \leq \mu_i, \qquad i=1, \ldots, C \label{eq4set}  \\
\alpha_{ij} &=& (1-A_{ij}) \lambda_{ij} + \left( \sum_{k=1}^C \alpha_{kj} q_{ki}(j) \right) \label{eq3set}   \\
A_{ij}& \in & \{ 0, 1 \}, \alpha_{ij} \in \mathbb{R}
\end{eqnarray}
The goal of the optimization is to minimize the amount of requests that require service in the network~\eqref{eqgoal}.
According to~\eqref{eq1set}, each file must be present in at least one cache.   Equatiosn ~\eqref{eq2set} and ~\eqref{eq4set}
 are  constraints on the size 
and service capacity
of the caches, respectively. Finally, ~\eqref{eq3set} are the flow balance equations.


The control variables are the integer valued $A_{ij}$, $i=1,\ldots, C$, $j=1, \ldots, F$.  	Since the auxiliary real variables 
$\alpha_{ij}$ are multiplied by $A_{ij}$, we have a quadratic constrained program.   Although mixed integer programming is NP hard, there are
 well known heuristics to solve such problems~\cite{miqcp} when the constraints are quadratic. \eat{ In~\textsection\ref{sec:eval} we rely on some of these
 heuristics to numerically evaluate solutions to the optimal content placement problem.} 



==> system.tex <==
\section{System: Data Plane and Control Plane}

The systems considered in this paper are cache networks.  Information flows in a cache network through two planes, the data plane and the 
control plane.  In the control plane caches exchange requests and routing informations, whereas the content moves in the data plane.

In this paper we consider a well provisioned data plane.  The data plane is not a bottleneck  and our focus is on the control plane.  
In particular, we assume that the data plane
 is always stable, i.e., once a content is found it will always be served in finite time.  Users are patient, and 
wait for their downloads to conclude.    
  \emph{Our aim is to analyze how content placement affects the stability 
region of the control plane.}  


Note that in systems where the data plane is not guaranteed to be well provisioned, the stability of the
control plane is necessary for the stability of the sytem as a whole.   Therefore, the results presented in this paper are also 
applicable to systems where the data plane is not guaranteed to be well provisioned.

The system considered in this paper is illustrated in Figure~\ref{system}.  A request for file $F$ is routed using random walks through
the caches.  Every time the request hits a cache, the cache selects uniformly at random one of the \eat{other} links that are incident to the cache
and uses it to forward the request.  Once the request reaches a cache where the content is stored, the content is transfered to the requester
through the data plane.


We assume that all contents are stored in at least one cache.  When devising content placement strategies in the forthcoming sections, we
 will enforce that this requirement is always satisfied.  

\begin{figure}
\begin{center}
\includegraphics[scale=0.20]{cache4} 
\end{center}
\caption{Illustration of how system works (cache-router symbol introduced in~\cite{breadcrumbs1}).  $(a)$ An exogenous request for file $F$ is placed and processed in cache 1;  $(b)$ the request is routed through the control plane, and yields an endogenous request  to cache 2; $(c)$ the request is processed in cache 2; $(d)$ the request is routed through the control plane to cache 4. The file is found and is transfered to the user through the data plane.}
\label{system}
\end{figure}

